A Vehicle System for Navigating Among Vulnerable Road Users Including Remote Operation

We present a vehicle system capable of navigating safely and efficiently around Vulnerable Road Users (VRUs), such as pedestrians and cyclists. The system comprises key modules for environment perception, localization and mapping, motion planning, and control, integrated into a prototype vehicle. A key innovation is a motion planner based on Topology-driven Model Predictive Control (T-MPC). The guidance layer generates multiple trajectories in parallel, each representing a distinct strategy for obstacle avoidance or non-passing. The underlying trajectory optimization constrains the joint probability of collision with VRUs under generic uncertainties. To address extraordinary situations ("edge cases") that go beyond the autonomous capabilities - such as construction zones or encounters with emergency responders - the system includes an option for remote human operation, supported by visual and haptic guidance. In simulation, our motion planner outperforms three baseline approaches in terms of safety and efficiency. We also demonstrate the full system in prototype vehicle tests on a closed track, both in autonomous and remotely operated modes.

==> 3_SelfDrivingSystem/c-Perception/perception_figure.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.95\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{7 Appendix/centerpoint.jpg}
        \caption{Object Detection}    
        \label{fig:perception_centerpoint}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.95\columnwidth}  
        \centering 
        \includegraphics[width=\textwidth]{7 Appendix/shape_estimation.jpg}
        \caption{LiDAR Clustering}    
        \label{fig:perception_clustering}
    \end{subfigure}
    \caption{
    A visualization of the outputs of the object detector and LiDAR clustering.
    (a) The object detector detects a predefined set of object classes (e.g. car and pedestrian).
    (b) The LiDAR clustering segments any object protruding from the ground plane, including generic objects.
    }
    \label{fig:perception_qualitative_results}
\end{figure*}

==> 3_SelfDrivingSystem/e-MotionPlanning/demo-2022-crossing.tex <==
% \begin{figure*}[h]
%     \captionsetup{justification=raggedright}
%     \centering
%     \begin{subfigure}[t]{0.3\textwidth}
%         \centering
%         % Answer: [trim={left bottom right top},clip]
%         % \includegraphics[width=\textwidth,trim={0cm 0cm 4cm 0.5cm},clip]{chapters/application/figures/demo-2022/Selection_887.png}
%         \includegraphics[width=\textwidth,trim={1cm 0cm 2cm 7.5cm},clip]{5 Demonstration/figures/Selection_889.png}
%         \caption{$t = 3$ s}
%         \label{fig:crossing-2022-screena}%%
%     \end{subfigure}
%     \hspace{0.01\textwidth}
%     \begin{subfigure}[t]{0.29\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={1cm 0cm 2cm 7.5cm},clip]{5 Demonstration/figures/Selection_887.png}
%         \caption{$t = 4$ s}
%         \label{fig:crossing-2022-screenb}%%
%     \end{subfigure}
%     \hspace{0.01\textwidth}
%     \begin{subfigure}[t]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={1cm 0cm 2cm 7.5cm},clip]{5 Demonstration/figures/Selection_888.png}
%         \caption{$t = 8$ s}
%         \label{fig:crossing-2022-screenc}%%
%     \end{subfigure}

%     \begin{subfigure}[t]{0.9\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{5 Demonstration/figures/trajectories_crossing.pdf}
%         \caption{Vehicle trajectory.}
%         \label{fig:crossing-2022-trajectories}%%
%     \end{subfigure}
%     \caption{(a-c) Screenshot of the dynamic demonstration of Scenario~3 using SH-MPC. The planned trajectory evades a crossing pedestrian. Visualized are samples of the pedestrian's trajectory (dotted lines), support samples (solid circles) and probabilistic polytopes from blue (stage $1$) to green (stage $19$).}
%     \label{fig:crossing-2022}
% \end{figure*}
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{3 Self-Driving System/e - Motion Planning/dense-4.pdf}
    \caption{\oscar{Snapshot of the motion planner navigating among virtual VRUs. Sampled VRU predictions and probabilistic safe polytopes are denoted from blue (stage $1$) to green (stage $29$). Blue circles show the planned trajectory.}}
    \label{fig:crossing-2022}
\end{figure}


==> 5_Experiments/demo-2022-headon.tex <==
\begin{figure*}[h]
    \captionsetup{justification=raggedright}
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={14cm 5cm 0cm 7cm},clip]{5 Demonstration/figures/Selection_893.png}
        \caption{$t = 5$ s}
        \label{fig:headon-2022-screena}%%
    \end{subfigure}
    \hspace{0.01\textwidth}
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={14cm 5cm 0cm 7cm},clip]{5 Demonstration/figures/Selection_891.png}
        \caption{$t = 6$ s}
        \label{fig:headon-2022-screenb}%%
    \end{subfigure}
    \hspace{0.01\textwidth}
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={14cm 5cm 0cm 7cm},clip]{5 Demonstration/figures/Selection_892.png}
        \caption{$t = 9$ s}
        \label{fig:headon-2022-screenc}%%
    \end{subfigure}

    \begin{subfigure}[t]{0.9\textwidth}
        \centering
        \includegraphics[width=\textwidth]{5 Demonstration/figures/trajectories_headon.pdf}
        \caption{Vehicle trajectory.}
        \label{fig:headon-2022-trajectories}%%
    \end{subfigure}
    \caption{Visualizations (similar to Fig.~\ref{fig:crossing-2022}) for a head-on encounter.}
    \label{fig:headon-2022}
\end{figure*}
